Solving Some Geometry Problems of the N\'aboj 2023 Contest with Automated Deduction in GeoGebra Discovery

In this article, we solve some of the geometry problems of the N\'aboj 2023 competition with the help of a computer, using examples that the software tool GeoGebra Discovery can calculate. In each case, the calculation requires symbolic computations. We analyze the difficulty of feeding the problem into the machine and set further goals to make the problems of this type of contests even more tractable in the future.

==> eptcsdata.tex <==
\providecommand{\firstpage}{110}
\providecommand{\publicationstatus}{P. Quaresma and Z. Kov{\'a}cs (Ed.): Automated Deduction\\ in Geometry 2023 (ADG 2023).\\
EPTCS 398, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.398.14}{10.4204/EPTCS.398.14}}
\pdfoutput=1

